Vector incremental treatment effects

Causal questions involving multiple binary treatments are poorly served by standard causal approaches. Potential outcomes grow exponentially with the number of treatments, many treatment combinations are rarely or never observed, and fixing everyone to one combination can require implausible positivity assumptions. We extend incremental propensity score interventions to vector-valued binary treatments, defining causal effects through counterfactual distributions that scale the odds of each treatment by a user-specified factor. Because marginal odds constraints do not uniquely determine the joint distribution, we define it as the minimum-divergence projection of the observed law onto the constrained set, for a user-specified separable divergence, preserving the observed conditional support. The resulting counterfactual mean outcome is identified under consistency and conditional mean exchangeability, without requiring every treatment combination to have positive conditional probability. For a class of smooth divergences, we derive the efficient influence function and construct cross-fitted one-step estimators that are consistent at the parametric rate and asymptotically normal when marginal treatment probabilities are exactly 0, exactly 1, or bounded away from those values. We relax this requirement by specifying a different estimand and deriving a corresponding estimator, which is asymptotically normal under a convergence-rate condition on the estimated active set. We also extend sensitivity analysis to address unmeasured confounding. Applying the framework to 159,466 New York Medicaid beneficiaries with serious mental illness, we estimate how healthcare costs would change under uniform improvements in the odds of six recommended quality-of-care processes. Increasing recommended care is associated with lower total, inpatient, and mental-health cost and higher outpatient cost.

==> common-defs.tex <==

\ProvidesPackage{common_definitions}[2025/06/10 Common mathematical definitions]


\DeclareMathOperator{\Tr}{Tr}           
\DeclareMathOperator{\rank}{rank}       
\DeclareMathOperator{\spn}{span}        
\DeclareMathOperator{\im}{im}           
\DeclareMathOperator{\coker}{coker}     
\DeclareMathOperator{\supp}{supp}       
\DeclareMathOperator{\diag}{diag}       

\DeclareMathOperator{\grad}{grad}       
\DeclareMathOperator{\divop}{div}       
\DeclareMathOperator{\curl}{curl}       
\DeclareMathOperator{\sign}{sign}       
\DeclareMathOperator{\sinc}{sinc}       

\DeclareMathOperator{\Var}{Var}         
\DeclareMathOperator{\Cov}{Cov}         
\DeclareMathOperator{\Corr}{Corr}       
\DeclareMathOperator{\Bias}{Bias}       
\DeclareMathOperator{\MSE}{MSE}         
\DeclareMathOperator*{\argmin}{arg\,min} 
\DeclareMathOperator*{\argmax}{arg\,max} 

\DeclareMathOperator{\prox}{prox}       
\DeclareMathOperator{\proj}{proj}       


\newcommand{\ba}{\mathbf{a}}            \newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}            \newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}            \newcommand{\bff}{\mathbf{f}}           
\newcommand{\bg}{\mathbf{g}}            \newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}            \newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}            \newcommand{\bl}{\mathbf{l}}
\newcommand{\bm}{\mathbf{m}}            \newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}            \newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}            \newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}            \newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}            \newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}            \newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}            \newcommand{\bz}{\mathbf{z}}

\newcommand{\bA}{\mathbf{A}}            \newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}            \newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}            \newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}            \newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}            \newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}            \newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}            \newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}            \newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}            \newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}            \newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}            \newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}            \newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}            \newcommand{\bZ}{\mathbf{Z}}

\newcommand{\balpha}{\boldsymbol{\alpha}}       \newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}       \newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}   \newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bfeta}{\boldsymbol{\eta}}          \newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\biota}{\boldsymbol{\iota}}         \newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}     \newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}             \newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bomicron}{\boldsymbol{\omicron}}   \newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\brho}{\boldsymbol{\rho}}           \newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}           \newcommand{\bupsilon}{\boldsymbol{\upsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}           \newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}           \newcommand{\bomega}{\boldsymbol{\omega}}

\newcommand{\bGamma}{\boldsymbol{\Gamma}}       \newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}       \newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bXi}{\boldsymbol{\Xi}}             \newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}       \newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}           \newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

\newcommand{\A}{\mathbb{A}}             \newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}}             \newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}             \newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}             \newcommand{\bboardH}{\mathbb{H}}
\newcommand{\I}{\mathbb{I}}             \newcommand{\J}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}             \newcommand{\bboardL}{\mathbb{L}}
\newcommand{\M}{\mathbb{M}}             \newcommand{\N}{\mathbb{N}}
\newcommand{\bboardO}{\mathbb{O}}       \newcommand{\bboardP}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}             \newcommand{\R}{\mathbb{R}}
\newcommand{\bboardS}{\mathbb{S}}       \newcommand{\T}{\mathbb{T}}
\newcommand{\U}{\mathbb{U}}             \newcommand{\V}{\mathbb{V}}
\newcommand{\W}{\mathbb{W}}             \newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}             \newcommand{\Z}{\mathbb{Z}}

\newcommand{\cA}{\mathcal{A}}           \newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}           \newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}           \newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}           \newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}           \newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}           \newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}           \newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}           \newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}           \newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}           \newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}           \newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}           \newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}           \newcommand{\cZ}{\mathcal{Z}}



\newcommand{\Rn}{\R^n}                  
\newcommand{\Rm}{\R^m}                  
\newcommand{\Rd}{\R^d}                  
\newcommand{\Cn}{\C^n}                  

\newcommand{\Lp}[1]{L^{#1}}             
\newcommand{\Lone}{L^1}                 
\newcommand{\Ltwo}{L^2}                 
\newcommand{\Linf}{L^\infty}            
\newcommand{\Ck}[1]{C^{#1}}             
\newcommand{\Cinf}{C^\infty}            


\newcommand{\Prob}{\bboardP}             

\newcommand{\Normal}{\cN}               
\newcommand{\Unif}{\mathrm{Unif}}       
\newcommand{\Bern}{\mathrm{Bern}}       
\newcommand{\Binom}{\mathrm{Binom}}     
\newcommand{\Pois}{\mathrm{Pois}}       


\newcommand{\norm}[1]{\left\|#1\right\|}           
\newcommand{\abs}[1]{\left|#1\right|}              
\newcommand{\inner}[2]{\left\langle#1,#2\right\rangle} 
\newcommand{\pnorm}[2]{\|#1\|_{#2}}                
\newcommand{\onenorm}[1]{\|#1\|_1}                 
\newcommand{\twonorm}[1]{\|#1\|_2}                 
\newcommand{\infnorm}[1]{\|#1\|_\infty}           
\newcommand{\fronorm}[1]{\|#1\|_F}                 


\newcommand{\paren}[1]{\left(#1\right)}            
\newcommand{\bracket}[1]{\left[#1\right]}          
\newcommand{\setbrace}[1]{\left\{#1\right\}}        
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor} 
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}   


\newcommand{\dx}{\,dx}                  
\newcommand{\dy}{\,dy}                  
\newcommand{\dt}{\,dt}                  
\newcommand{\du}{\,du}                  
\newcommand{\dv}{\,dv}                  

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}       
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}} 
\newcommand{\pdmixed}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}} 

\newcommand{\dd}[2]{\frac{d #1}{d #2}}                     
\newcommand{\ddd}[2]{\frac{d^2 #1}{d #2^2}}               


\newcommand{\transpose}[1]{#1^T}        
\newcommand{\hermitian}[1]{#1^*}        
\newcommand{\inv}[1]{#1^{-1}}           
\newcommand{\pinv}[1]{#1^{\dagger}}     

\newcommand{\mat}[1]{\mathbf{#1}}       
\newcommand{\vect}[1]{\mathbf{#1}}      
\newcommand{\vzero}{\mathbf{0}}         
\newcommand{\vone}{\mathbf{1}}          
\newcommand{\eye}{\mathbf{I}}           


\newcommand{\bigO}{\cO}                 
\newcommand{\smallO}{\mathrm{o}}        
\newcommand{\bigOmega}{\Omega}          
\newcommand{\smallOmega}{\omega}        
\newcommand{\bigTheta}{\Theta}          


\newcommand{\diam}{\mathrm{diam}}       
\newcommand{\iid}{\text{i.i.d.}}        
\newcommand{\as}{\text{a.s.}}           
\newcommand{\aeq}{\text{a.e.}}           
\newcommand{\wrt}{\text{w.r.t.}}        
\newcommand{\suchthat}{\text{s.t.}}     
\newcommand{\defn}{\coloneqq}           
\newcommand{\indep}{\perp\!\!\!\perp}   


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}







\newcommand{\ahat}{\hat{a}}             \newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}             \newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}             \newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}             \newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}             \newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}             \newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}             \newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}             \newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}             \newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}             \newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}             \newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}             \newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}             \newcommand{\zhat}{\hat{z}}

\newcommand{\Ahat}{\hat{A}}             \newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}             \newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}             \newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}             \newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}             \newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}             \newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}             \newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}             \newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}             \newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}             \newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}             \newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}             \newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}             \newcommand{\Zhat}{\hat{Z}}

\newcommand{\alphahat}{\hat{\alpha}}    \newcommand{\betahat}{\hat{\beta}}
\newcommand{\gammahat}{\hat{\gamma}}    \newcommand{\deltahat}{\hat{\delta}}
\newcommand{\epsilonhat}{\hat{\epsilon}} \newcommand{\varepsilonhat}{\hat{\varepsilon}}
\newcommand{\zetahat}{\hat{\zeta}}      \newcommand{\etahat}{\hat{\eta}}
\newcommand{\thetahat}{\hat{\theta}}    \newcommand{\varthetahat}{\hat{\vartheta}}
\newcommand{\iotahat}{\hat{\iota}}      \newcommand{\kappahat}{\hat{\kappa}}
\newcommand{\lambdahat}{\hat{\lambda}}  \newcommand{\muhat}{\hat{\mu}}
\newcommand{\nuhat}{\hat{\nu}}          \newcommand{\xihat}{\hat{\xi}}
\newcommand{\omicronhat}{\hat{\omicron}} \newcommand{\pihat}{\hat{\pi}}
\newcommand{\varpihat}{\hat{\varpi}}    \newcommand{\rhohat}{\hat{\rho}}
\newcommand{\varrhohat}{\hat{\varrho}}  \newcommand{\sigmahat}{\hat{\sigma}}
\newcommand{\varsigmahat}{\hat{\varsigma}} \newcommand{\tauhat}{\hat{\tau}}
\newcommand{\upsilonhat}{\hat{\upsilon}} \newcommand{\phihat}{\hat{\phi}}
\newcommand{\varphihat}{\hat{\varphi}}  \newcommand{\chihat}{\hat{\chi}}
\newcommand{\psihat}{\hat{\psi}}        \newcommand{\omegahat}{\hat{\omega}}

\newcommand{\Gammahat}{\hat{\Gamma}}    \newcommand{\Deltahat}{\hat{\Delta}}
\newcommand{\Thetahat}{\hat{\Theta}}    \newcommand{\Lambdahat}{\hat{\Lambda}}
\newcommand{\Xihat}{\hat{\Xi}}          \newcommand{\Pihat}{\hat{\Pi}}
\newcommand{\Sigmahat}{\hat{\Sigma}}    \newcommand{\Upsilonhat}{\hat{\Upsilon}}
\newcommand{\Phihat}{\hat{\Phi}}        \newcommand{\Psihat}{\hat{\Psi}}
\newcommand{\Omegahat}{\hat{\Omega}}

\newcommand{\bahat}{\hat{\ba}}          \newcommand{\bbhat}{\hat{\bb}}
\newcommand{\bchat}{\hat{\bc}}          \newcommand{\bdhat}{\hat{\bd}}
\newcommand{\behat}{\hat{\be}}          \newcommand{\bfhat}{\hat{\bff}}
\newcommand{\bghat}{\hat{\bg}}          \newcommand{\bhhat}{\hat{\bh}}
\newcommand{\bihat}{\hat{\bi}}          \newcommand{\bjhat}{\hat{\bj}}
\newcommand{\bkhat}{\hat{\bk}}          \newcommand{\blhat}{\hat{\bl}}
\newcommand{\bmhat}{\hat{\bm}}          \newcommand{\bnhat}{\hat{\bn}}
\newcommand{\bohat}{\hat{\bo}}          \newcommand{\bphat}{\hat{\bp}}
\newcommand{\bqhat}{\hat{\bq}}          \newcommand{\brhat}{\hat{\br}}
\newcommand{\bshat}{\hat{\bs}}          \newcommand{\bthat}{\hat{\bt}}
\newcommand{\buhat}{\hat{\bu}}          \newcommand{\bvhat}{\hat{\bv}}
\newcommand{\bwhat}{\hat{\bw}}          \newcommand{\bxhat}{\hat{\bx}}
\newcommand{\byhat}{\hat{\by}}          \newcommand{\bzhat}{\hat{\bz}}

\newcommand{\bAhat}{\hat{\bA}}          \newcommand{\bBhat}{\hat{\bB}}
\newcommand{\bChat}{\hat{\bC}}          \newcommand{\bDhat}{\hat{\bD}}
\newcommand{\bEhat}{\hat{\bE}}          \newcommand{\bFhat}{\hat{\bF}}
\newcommand{\bGhat}{\hat{\bG}}          \newcommand{\bHhat}{\hat{\bH}}
\newcommand{\bIhat}{\hat{\bI}}          \newcommand{\bJhat}{\hat{\bJ}}
\newcommand{\bKhat}{\hat{\bK}}          \newcommand{\bLhat}{\hat{\bL}}
\newcommand{\bMhat}{\hat{\bM}}          \newcommand{\bNhat}{\hat{\bN}}
\newcommand{\bOhat}{\hat{\bO}}          \newcommand{\bPhat}{\hat{\bP}}
\newcommand{\bQhat}{\hat{\bQ}}          \newcommand{\bRhat}{\hat{\bR}}
\newcommand{\bShat}{\hat{\bS}}          \newcommand{\bThat}{\hat{\bT}}
\newcommand{\bUhat}{\hat{\bU}}          \newcommand{\bVhat}{\hat{\bV}}
\newcommand{\bWhat}{\hat{\bW}}          \newcommand{\bXhat}{\hat{\bX}}
\newcommand{\bYhat}{\hat{\bY}}          \newcommand{\bZhat}{\hat{\bZ}}

\newcommand{\balphahat}{\hat{\balpha}}  \newcommand{\bbetahat}{\hat{\bbeta}}
\newcommand{\bgammahat}{\hat{\bgamma}}  \newcommand{\bdeltahat}{\hat{\bdelta}}
\newcommand{\bepsilonhat}{\hat{\bepsilon}} \newcommand{\bzetahat}{\hat{\bzeta}}
\newcommand{\bfetahat}{\hat{\bfeta}}    \newcommand{\bthetahat}{\hat{\btheta}}
\newcommand{\biotahat}{\hat{\biota}}    \newcommand{\bkappahat}{\hat{\bkappa}}
\newcommand{\blambdahat}{\hat{\blambda}} \newcommand{\bmuhat}{\hat{\bmu}}
\newcommand{\bnuhat}{\hat{\bnu}}        \newcommand{\bxihat}{\hat{\bxi}}
\newcommand{\bpihat}{\hat{\bpi}}        \newcommand{\brhohat}{\hat{\brho}}
\newcommand{\bsigmahat}{\hat{\bsigma}}  \newcommand{\btauhat}{\hat{\btau}}
\newcommand{\bupsilonhat}{\hat{\bupsilon}} \newcommand{\bphihat}{\hat{\bphi}}
\newcommand{\bchihat}{\hat{\bchi}}      \newcommand{\bpsihat}{\hat{\bpsi}}
\newcommand{\bomegahat}{\hat{\bomega}}

\newcommand{\bGammahat}{\hat{\bGamma}}  \newcommand{\bDeltahat}{\hat{\bDelta}}
\newcommand{\bThetahat}{\hat{\bTheta}}  \newcommand{\bLambdahat}{\hat{\bLambda}}
\newcommand{\bXihat}{\hat{\bXi}}        \newcommand{\bPihat}{\hat{\bPi}}
\newcommand{\bSigmahat}{\hat{\bSigma}}  \newcommand{\bUpsilonhat}{\hat{\bUpsilon}}
\newcommand{\bPhihat}{\hat{\bPhi}}      \newcommand{\bPsihat}{\hat{\bPsi}}
\newcommand{\bOmegahat}{\hat{\bOmega}}


\newcommand{\atilde}{\tilde{a}}         \newcommand{\btilde}{\tilde{b}}
\newcommand{\ctilde}{\tilde{c}}         \newcommand{\dtilde}{\tilde{d}}
\newcommand{\etilde}{\tilde{e}}         \newcommand{\ftilde}{\tilde{f}}
\newcommand{\gtilde}{\tilde{g}}         \newcommand{\htilde}{\tilde{h}}
\newcommand{\itilde}{\tilde{i}}         \newcommand{\jtilde}{\tilde{j}}
\newcommand{\ktilde}{\tilde{k}}         \newcommand{\ltilde}{\tilde{l}}
\newcommand{\mtilde}{\tilde{m}}         \newcommand{\ntilde}{\tilde{n}}
\newcommand{\otilde}{\tilde{o}}         \newcommand{\ptilde}{\tilde{p}}
\newcommand{\qtilde}{\tilde{q}}         \newcommand{\rtilde}{\tilde{r}}
\newcommand{\stilde}{\tilde{s}}         \newcommand{\ttilde}{\tilde{t}}
\newcommand{\utilde}{\tilde{u}}         \newcommand{\vtilde}{\tilde{v}}
\newcommand{\wtilde}{\tilde{w}}         \newcommand{\xtilde}{\tilde{x}}
\newcommand{\ytilde}{\tilde{y}}         \newcommand{\ztilde}{\tilde{z}}

\newcommand{\Atilde}{\tilde{A}}         \newcommand{\Btilde}{\tilde{B}}
\newcommand{\Ctilde}{\tilde{C}}         \newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Etilde}{\tilde{E}}         \newcommand{\Ftilde}{\tilde{F}}
\newcommand{\Gtilde}{\tilde{G}}         \newcommand{\Htilde}{\tilde{H}}
\newcommand{\Itilde}{\tilde{I}}         \newcommand{\Jtilde}{\tilde{J}}
\newcommand{\Ktilde}{\tilde{K}}         \newcommand{\Ltilde}{\tilde{L}}
\newcommand{\Mtilde}{\tilde{M}}         \newcommand{\Ntilde}{\tilde{N}}
\newcommand{\Otilde}{\tilde{O}}         \newcommand{\Ptilde}{\tilde{P}}
\newcommand{\Qtilde}{\tilde{Q}}         \newcommand{\Rtilde}{\tilde{R}}
\newcommand{\Stilde}{\tilde{S}}         \newcommand{\Ttilde}{\tilde{T}}
\newcommand{\Utilde}{\tilde{U}}         \newcommand{\Vtilde}{\tilde{V}}
\newcommand{\Wtilde}{\tilde{W}}         \newcommand{\Xtilde}{\tilde{X}}
\newcommand{\Ytilde}{\tilde{Y}}         \newcommand{\Ztilde}{\tilde{Z}}

\newcommand{\alphatilde}{\tilde{\alpha}} \newcommand{\betatilde}{\tilde{\beta}}
\newcommand{\gammatilde}{\tilde{\gamma}} \newcommand{\deltatilde}{\tilde{\delta}}
\newcommand{\epsilontilde}{\tilde{\epsilon}} \newcommand{\varepsilontilde}{\tilde{\varepsilon}}
\newcommand{\zetatilde}{\tilde{\zeta}}  \newcommand{\etatilde}{\tilde{\eta}}
\newcommand{\thetatilde}{\tilde{\theta}} \newcommand{\varthetatilde}{\tilde{\vartheta}}
\newcommand{\iotatilde}{\tilde{\iota}}  \newcommand{\kappatilde}{\tilde{\kappa}}
\newcommand{\lambdatilde}{\tilde{\lambda}} \newcommand{\mutilde}{\tilde{\mu}}
\newcommand{\nutilde}{\tilde{\nu}}      \newcommand{\xitilde}{\tilde{\xi}}
\newcommand{\omicrontilde}{\tilde{\omicron}} \newcommand{\pitilde}{\tilde{\pi}}
\newcommand{\varpitilde}{\tilde{\varpi}} \newcommand{\rhotilde}{\tilde{\rho}}
\newcommand{\varrhotilde}{\tilde{\varrho}} \newcommand{\sigmatilde}{\tilde{\sigma}}
\newcommand{\varsigmatilde}{\tilde{\varsigma}} \newcommand{\tautilde}{\tilde{\tau}}
\newcommand{\upsilontilde}{\tilde{\upsilon}} \newcommand{\phitilde}{\tilde{\phi}}
\newcommand{\varphitilde}{\tilde{\varphi}} \newcommand{\chitilde}{\tilde{\chi}}
\newcommand{\psitilde}{\tilde{\psi}}    \newcommand{\omegatilde}{\tilde{\omega}}

\newcommand{\Gammatilde}{\tilde{\Gamma}} \newcommand{\Deltatilde}{\tilde{\Delta}}
\newcommand{\Thetatilde}{\tilde{\Theta}} \newcommand{\Lambdatilde}{\tilde{\Lambda}}
\newcommand{\Xitilde}{\tilde{\Xi}}      \newcommand{\Pitilde}{\tilde{\Pi}}
\newcommand{\Sigmatilde}{\tilde{\Sigma}} \newcommand{\Upsilontilde}{\tilde{\Upsilon}}
\newcommand{\Phitilde}{\tilde{\Phi}}    \newcommand{\Psitilde}{\tilde{\Psi}}
\newcommand{\Omegatilde}{\tilde{\Omega}}

\newcommand{\batilde}{\tilde{\ba}}      \newcommand{\bbtilde}{\tilde{\bb}}
\newcommand{\bctilde}{\tilde{\bc}}      \newcommand{\bdtilde}{\tilde{\bd}}
\newcommand{\betilde}{\tilde{\be}}      \newcommand{\bftilde}{\tilde{\bff}}
\newcommand{\bgtilde}{\tilde{\bg}}      \newcommand{\bhtilde}{\tilde{\bh}}
\newcommand{\bitilde}{\tilde{\bi}}      \newcommand{\bjtilde}{\tilde{\bj}}
\newcommand{\bktilde}{\tilde{\bk}}      \newcommand{\bltilde}{\tilde{\bl}}
\newcommand{\bmtilde}{\tilde{\bm}}      \newcommand{\bntilde}{\tilde{\bn}}
\newcommand{\botilde}{\tilde{\bo}}      \newcommand{\bptilde}{\tilde{\bp}}
\newcommand{\bqtilde}{\tilde{\bq}}      \newcommand{\brtilde}{\tilde{\br}}
\newcommand{\bstilde}{\tilde{\bs}}      \newcommand{\bttilde}{\tilde{\bt}}
\newcommand{\butilde}{\tilde{\bu}}      \newcommand{\bvtilde}{\tilde{\bv}}
\newcommand{\bwtilde}{\tilde{\bw}}      \newcommand{\bxtilde}{\tilde{\bx}}
\newcommand{\bytilde}{\tilde{\by}}      \newcommand{\bztilde}{\tilde{\bz}}

\newcommand{\bAtilde}{\tilde{\bA}}      \newcommand{\bBtilde}{\tilde{\bB}}
\newcommand{\bCtilde}{\tilde{\bC}}      \newcommand{\bDtilde}{\tilde{\bD}}
\newcommand{\bEtilde}{\tilde{\bE}}      \newcommand{\bFtilde}{\tilde{\bF}}
\newcommand{\bGtilde}{\tilde{\bG}}      \newcommand{\bHtilde}{\tilde{\bH}}
\newcommand{\bItilde}{\tilde{\bI}}      \newcommand{\bJtilde}{\tilde{\bJ}}
\newcommand{\bKtilde}{\tilde{\bK}}      \newcommand{\bLtilde}{\tilde{\bL}}
\newcommand{\bMtilde}{\tilde{\bM}}      \newcommand{\bNtilde}{\tilde{\bN}}
\newcommand{\bOtilde}{\tilde{\bO}}      \newcommand{\bPtilde}{\tilde{\bP}}
\newcommand{\bQtilde}{\tilde{\bQ}}      \newcommand{\bRtilde}{\tilde{\bR}}
\newcommand{\bStilde}{\tilde{\bS}}      \newcommand{\bTtilde}{\tilde{\bT}}
\newcommand{\bUtilde}{\tilde{\bU}}      \newcommand{\bVtilde}{\tilde{\bV}}
\newcommand{\bWtilde}{\tilde{\bW}}      \newcommand{\bXtilde}{\tilde{\bX}}
\newcommand{\bYtilde}{\tilde{\bY}}      \newcommand{\bZtilde}{\tilde{\bZ}}

\newcommand{\balphatilde}{\tilde{\balpha}} \newcommand{\bbetatilde}{\tilde{\bbeta}}
\newcommand{\bgammatilde}{\tilde{\bgamma}} \newcommand{\bdeltatilde}{\tilde{\bdelta}}
\newcommand{\bepsilontilde}{\tilde{\bepsilon}} \newcommand{\bzetatilde}{\tilde{\bzeta}}
\newcommand{\bfetatilde}{\tilde{\bfeta}} \newcommand{\bthetatilde}{\tilde{\btheta}}
\newcommand{\biotatilde}{\tilde{\biota}} \newcommand{\bkappatilde}{\tilde{\bkappa}}
\newcommand{\blambdatilde}{\tilde{\blambda}} \newcommand{\bmutilde}{\tilde{\bmu}}
\newcommand{\bnutilde}{\tilde{\bnu}}    \newcommand{\bxitilde}{\tilde{\bxi}}
\newcommand{\bpitilde}{\tilde{\bpi}}    \newcommand{\brhotilde}{\tilde{\brho}}
\newcommand{\bsigmatilde}{\tilde{\bsigma}} \newcommand{\btautilde}{\tilde{\btau}}
\newcommand{\bupsilontilde}{\tilde{\bupsilon}} \newcommand{\bphitilde}{\tilde{\bphi}}
\newcommand{\bchitilde}{\tilde{\bchi}}  \newcommand{\bpsitilde}{\tilde{\bpsi}}
\newcommand{\bomegatilde}{\tilde{\bomega}}

\newcommand{\bGammatilde}{\tilde{\bGamma}} \newcommand{\bDeltatilde}{\tilde{\bDelta}}
\newcommand{\bThetatilde}{\tilde{\bTheta}} \newcommand{\bLambdatilde}{\tilde{\bLambda}}
\newcommand{\bXitilde}{\tilde{\bXi}}    \newcommand{\bPitilde}{\tilde{\bPi}}
\newcommand{\bSigmatilde}{\tilde{\bSigma}} \newcommand{\bUpsilontilde}{\tilde{\bUpsilon}}
\newcommand{\bPhitilde}{\tilde{\bPhi}}

\newcommand{\abar}{\bar{a}}             \newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}             \newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}             \newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}             \newcommand{\barh}{\bar{h}}  
\newcommand{\ibar}{\bar{i}}             \newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}             \newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}             \newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}             \newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}             \newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}             \newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}             \newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}             \newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}             \newcommand{\zbar}{\bar{z}}

\newcommand{\Abar}{\bar{A}}             \newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}             \newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}             \newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}             \newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}             \newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}             \newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}             \newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}             \newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}             \newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}             \newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}             \newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}             \newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}             \newcommand{\Zbar}{\bar{Z}}

\newcommand{\alphabar}{\bar{\alpha}}    \newcommand{\betabar}{\bar{\beta}}
\newcommand{\gammabar}{\bar{\gamma}}    \newcommand{\deltabar}{\bar{\delta}}
\newcommand{\epsilonbar}{\bar{\epsilon}} \newcommand{\varepsilonbar}{\bar{\varepsilon}}
\newcommand{\zetabar}{\bar{\zeta}}      \newcommand{\etabar}{\bar{\eta}}
\newcommand{\thetabar}{\bar{\theta}}    \newcommand{\varthetabar}{\bar{\vartheta}}
\newcommand{\iotabar}{\bar{\iota}}      \newcommand{\kappabar}{\bar{\kappa}}
\newcommand{\lambdabar}{\bar{\lambda}}  \newcommand{\mubar}{\bar{\mu}}
\newcommand{\nubar}{\bar{\nu}}          \newcommand{\xibar}{\bar{\xi}}
\newcommand{\omicronbar}{\bar{\omicron}} \newcommand{\pibar}{\bar{\pi}}
\newcommand{\varpibar}{\bar{\varpi}}    \newcommand{\rhobar}{\bar{\rho}}
\newcommand{\varrhobar}{\bar{\varrho}}  \newcommand{\sigmabar}{\bar{\sigma}}
\newcommand{\varsigmabar}{\bar{\varsigma}} \newcommand{\taubar}{\bar{\tau}}
\newcommand{\upsilonbar}{\bar{\upsilon}} \newcommand{\phibar}{\bar{\phi}}
\newcommand{\varphibar}{\bar{\varphi}}  \newcommand{\chibar}{\bar{\chi}}
\newcommand{\psibar}{\bar{\psi}}        \newcommand{\omegabar}{\bar{\omega}}

\newcommand{\Gammabar}{\bar{\Gamma}}    \newcommand{\Deltabar}{\bar{\Delta}}
\newcommand{\Thetabar}{\bar{\Theta}}    \newcommand{\Lambdabar}{\bar{\Lambda}}
\newcommand{\Xibar}{\bar{\Xi}}          \newcommand{\Pibar}{\bar{\Pi}}
\newcommand{\Sigmabar}{\bar{\Sigma}}    \newcommand{\Upsilonbar}{\bar{\Upsilon}}
\newcommand{\Phibar}{\bar{\Phi}}        \newcommand{\Psibar}{\bar{\Psi}}
\newcommand{\Omegabar}{\bar{\Omega}}

\newcommand{\babar}{\bar{\ba}}          \newcommand{\bbbar}{\bar{\bb}}
\newcommand{\bcbar}{\bar{\bc}}          \newcommand{\bdbar}{\bar{\bd}}
\newcommand{\bebar}{\bar{\be}}          \newcommand{\bfbar}{\bar{\bff}}
\newcommand{\bgbar}{\bar{\bg}}          \newcommand{\bhbar}{\bar{\bh}}
\newcommand{\bibar}{\bar{\bi}}          \newcommand{\bjbar}{\bar{\bj}}
\newcommand{\bkbar}{\bar{\bk}}          \newcommand{\blbar}{\bar{\bl}}
\newcommand{\bmbar}{\bar{\bm}}          \newcommand{\bnbar}{\bar{\bn}}
\newcommand{\bobar}{\bar{\bo}}          \newcommand{\bpbar}{\bar{\bp}}
\newcommand{\bqbar}{\bar{\bq}}          \newcommand{\brbar}{\bar{\br}}
\newcommand{\bsbar}{\bar{\bs}}          \newcommand{\btbar}{\bar{\bt}}
\newcommand{\bubar}{\bar{\bu}}          \newcommand{\bvbar}{\bar{\bv}}
\newcommand{\bwbar}{\bar{\bw}}          \newcommand{\bxbar}{\bar{\bx}}
\newcommand{\bybar}{\bar{\by}}          \newcommand{\bzbar}{\bar{\bz}}

\newcommand{\bAbar}{\bar{\bA}}          \newcommand{\bBbar}{\bar{\bB}}
\newcommand{\bCbar}{\bar{\bC}}          \newcommand{\bDbar}{\bar{\bD}}
\newcommand{\bEbar}{\bar{\bE}}          \newcommand{\bFbar}{\bar{\bF}}
\newcommand{\bGbar}{\bar{\bG}}          \newcommand{\bHbar}{\bar{\bH}}
\newcommand{\bIbar}{\bar{\bI}}          \newcommand{\bJbar}{\bar{\bJ}}
\newcommand{\bKbar}{\bar{\bK}}          \newcommand{\bLbar}{\bar{\bL}}
\newcommand{\bMbar}{\bar{\bM}}          \newcommand{\bNbar}{\bar{\bN}}
\newcommand{\bObar}{\bar{\bO}}          \newcommand{\bPbar}{\bar{\bP}}
\newcommand{\bQbar}{\bar{\bQ}}          \newcommand{\bRbar}{\bar{\bR}}
\newcommand{\bSbar}{\bar{\bS}}          \newcommand{\bTbar}{\bar{\bT}}
\newcommand{\bUbar}{\bar{\bU}}          \newcommand{\bVbar}{\bar{\bV}}
\newcommand{\bWbar}{\bar{\bW}}          \newcommand{\bXbar}{\bar{\bX}}
\newcommand{\bYbar}{\bar{\bY}}          \newcommand{\bZbar}{\bar{\bZ}}

\newcommand{\balphabar}{\bar{\balpha}}  \newcommand{\bbetabar}{\bar{\bbeta}}
\newcommand{\bgammabar}{\bar{\bgamma}}  \newcommand{\bdeltabar}{\bar{\bdelta}}
\newcommand{\bepsilonbar}{\bar{\bepsilon}} \newcommand{\bzetabar}{\bar{\bzeta}}
\newcommand{\bfetabar}{\bar{\bfeta}}    \newcommand{\bthetabar}{\bar{\btheta}}
\newcommand{\biotabar}{\bar{\biota}}    \newcommand{\bkappabar}{\bar{\bkappa}}
\newcommand{\blambdabar}{\bar{\blambda}} \newcommand{\bmubar}{\bar{\bmu}}
\newcommand{\bnubar}{\bar{\bnu}}        \newcommand{\bxibar}{\bar{\bxi}}
\newcommand{\bpibar}{\bar{\bpi}}        \newcommand{\brhobar}{\bar{\brho}}
\newcommand{\bsigmabar}{\bar{\bsigma}}  \newcommand{\btaubar}{\bar{\btau}}
\newcommand{\bupsilonbar}{\bar{\bupsilon}} \newcommand{\bphibar}{\bar{\bphi}}
\newcommand{\bchibar}{\bar{\bchi}}      \newcommand{\bpsibar}{\bar{\bpsi}}
\newcommand{\bomegabar}{\bar{\bomega}}

\newcommand{\bGammabar}{\bar{\bGamma}}  \newcommand{\bDeltabar}{\bar{\bDelta}}
\newcommand{\bThetabar}{\bar{\bTheta}}  \newcommand{\bLambdabar}{\bar{\bLambda}}
\newcommand{\bXibar}{\bar{\bXi}}        \newcommand{\bPibar}{\bar{\bPi}}
\newcommand{\bSigmabar}{\bar{\bSigma}}  \newcommand{\bUpsilonbar}{\bar{\bUpsilon}}
\newcommand{\bPhibar}{\bar{\bPhi}}      \newcommand{\bPsibar}{\bar{\bPsi}}
\newcommand{\bOmegabar}{\bar{\bOmega}}

\newcommand{\aunderbar}{\underline{a}}          \newcommand{\bunderbar}{\underline{b}}
\newcommand{\cunderbar}{\underline{c}}          \newcommand{\dunderbar}{\underline{d}}
\newcommand{\eunderbar}{\underline{e}}          \newcommand{\funderbar}{\underline{f}}
\newcommand{\gunderbar}{\underline{g}}          \newcommand{\hunderbar}{\underline{h}}
\newcommand{\iunderbar}{\underline{i}}          \newcommand{\junderbar}{\underline{j}}
\newcommand{\kunderbar}{\underline{k}}          \newcommand{\lunderbar}{\underline{l}}
\newcommand{\munderbar}{\underline{m}}          \newcommand{\nunderbar}{\underline{n}}
\newcommand{\ounderbar}{\underline{o}}          \newcommand{\punderbar}{\underline{p}}
\newcommand{\qunderbar}{\underline{q}}          \newcommand{\runderbar}{\underline{r}}
\newcommand{\sunderbar}{\underline{s}}          \newcommand{\tunderbar}{\underline{t}}
\newcommand{\uunderbar}{\underline{u}}          \newcommand{\vunderbar}{\underline{v}}
\newcommand{\wunderbar}{\underline{w}}          \newcommand{\xunderbar}{\underline{x}}
\newcommand{\yunderbar}{\underline{y}}          \newcommand{\zunderbar}{\underline{z}}

\newcommand{\Aunderbar}{\underline{A}}          \newcommand{\Bunderbar}{\underline{B}}
\newcommand{\Cunderbar}{\underline{C}}          \newcommand{\Dunderbar}{\underline{D}}
\newcommand{\Eunderbar}{\underline{E}}          \newcommand{\Funderbar}{\underline{F}}
\newcommand{\Gunderbar}{\underline{G}}          \newcommand{\Hunderbar}{\underline{H}}
\newcommand{\Iunderbar}{\underline{I}}          \newcommand{\Junderbar}{\underline{J}}
\newcommand{\Kunderbar}{\underline{K}}          \newcommand{\Lunderbar}{\underline{L}}
\newcommand{\Munderbar}{\underline{M}}          \newcommand{\Nunderbar}{\underline{N}}
\newcommand{\Ounderbar}{\underline{O}}          \newcommand{\Punderbar}{\underline{P}}
\newcommand{\Qunderbar}{\underline{Q}}          \newcommand{\Runderbar}{\underline{R}}
\newcommand{\Sunderbar}{\underline{S}}          \newcommand{\Tunderbar}{\underline{T}}
\newcommand{\Uunderbar}{\underline{U}}          \newcommand{\Vunderbar}{\underline{V}}
\newcommand{\Wunderbar}{\underline{W}}          \newcommand{\Xunderbar}{\underline{X}}
\newcommand{\Yunderbar}{\underline{Y}}          \newcommand{\Zunderbar}{\underline{Z}}

\newcommand{\alphaunderbar}{\underline{\alpha}} \newcommand{\betaunderbar}{\underline{\beta}}
\newcommand{\gammaunderbar}{\underline{\gamma}} \newcommand{\deltaunderbar}{\underline{\delta}}
\newcommand{\epsilonunderbar}{\underline{\epsilon}} \newcommand{\varepsilonunderbar}{\underline{\varepsilon}}
\newcommand{\zetaunderbar}{\underline{\zeta}}    \newcommand{\etaunderbar}{\underline{\eta}}
\newcommand{\thetaunderbar}{\underline{\theta}} \newcommand{\varthetaunderbar}{\underline{\vartheta}}
\newcommand{\iotaunderbar}{\underline{\iota}}    \newcommand{\kappaunderbar}{\underline{\kappa}}
\newcommand{\lambdaunderbar}{\underline{\lambda}} \newcommand{\muunderbar}{\underline{\mu}}
\newcommand{\nuunderbar}{\underline{\nu}}        \newcommand{\xiunderbar}{\underline{\xi}}
\newcommand{\omicronunderbar}{\underline{\omicron}} \newcommand{\piunderbar}{\underline{\pi}}
\newcommand{\varpiunderbar}{\underline{\varpi}} \newcommand{\rhounderbar}{\underline{\rho}}
\newcommand{\varrhounderbar}{\underline{\varrho}} \newcommand{\sigmaunderbar}{\underline{\sigma}}
\newcommand{\varsigmaunderbar}{\underline{\varsigma}} \newcommand{\tauunderbar}{\underline{\tau}}
\newcommand{\upsilonunderbar}{\underline{\upsilon}} \newcommand{\phiunderbar}{\underline{\phi}}
\newcommand{\varphiunderbar}{\underline{\varphi}} \newcommand{\chiunderbar}{\underline{\chi}}
\newcommand{\psiunderbar}{\underline{\psi}}      \newcommand{\omegunderbar}{\underline{\omega}}

\newcommand{\Gammaunderbar}{\underline{\Gamma}} \newcommand{\Deltaunderbar}{\underline{\Delta}}
\newcommand{\Thetaunderbar}{\underline{\Theta}} \newcommand{\Lambdaunderbar}{\underline{\Lambda}}
\newcommand{\Xiunderbar}{\underline{\Xi}}        \newcommand{\Piunderbar}{\underline{\Pi}}
\newcommand{\Sigmaunderbar}{\underline{\Sigma}} \newcommand{\Upsilonunderbar}{\underline{\Upsilon}}
\newcommand{\Phiunderbar}{\underline{\Phi}}      \newcommand{\Psiunderbar}{\underline{\Psi}}
\newcommand{\Omegaunderbar}{\underline{\Omega}}

\newcommand{\baunderbar}{\underline{\ba}}       \newcommand{\bbunderbar}{\underline{\bb}}
\newcommand{\bcunderbar}{\underline{\bc}}       \newcommand{\bdunderbar}{\underline{\bd}}
\newcommand{\beunderbar}{\underline{\be}}       \newcommand{\bfunderbar}{\underline{\bff}}
\newcommand{\bgunderbar}{\underline{\bg}}       \newcommand{\bhunderbar}{\underline{\bh}}
\newcommand{\biunderbar}{\underline{\bi}}       \newcommand{\bjunderbar}{\underline{\bj}}
\newcommand{\bkunderbar}{\underline{\bk}}       \newcommand{\blunderbar}{\underline{\bl}}
\newcommand{\bmunderbar}{\underline{\bm}}       \newcommand{\bnunderbar}{\underline{\bn}}
\newcommand{\bounderbar}{\underline{\bo}}       \newcommand{\bpunderbar}{\underline{\bp}}
\newcommand{\bqunderbar}{\underline{\bq}}       \newcommand{\brunderbar}{\underline{\br}}
\newcommand{\bsunderbar}{\underline{\bs}}       \newcommand{\btunderbar}{\underline{\bt}}
\newcommand{\buunderbar}{\underline{\bu}}       \newcommand{\bvunderbar}{\underline{\bv}}
\newcommand{\bwunderbar}{\underline{\bw}}       \newcommand{\bxunderbar}{\underline{\bx}}
\newcommand{\byunderbar}{\underline{\by}}       \newcommand{\bzunderbar}{\underline{\bz}}

\newcommand{\bAunderbar}{\underline{\bA}}       \newcommand{\bBunderbar}{\underline{\bB}}
\newcommand{\bCunderbar}{\underline{\bC}}       \newcommand{\bDunderbar}{\underline{\bD}}
\newcommand{\bEunderbar}{\underline{\bE}}       \newcommand{\bFunderbar}{\underline{\bF}}
\newcommand{\bGunderbar}{\underline{\bG}}       \newcommand{\bHunderbar}{\underline{\bH}}
\newcommand{\bIunderbar}{\underline{\bI}}       \newcommand{\bJunderbar}{\underline{\bJ}}
\newcommand{\bKunderbar}{\underline{\bK}}       \newcommand{\bLunderbar}{\underline{\bL}}
\newcommand{\bMunderbar}{\underline{\bM}}       \newcommand{\bNunderbar}{\underline{\bN}}
\newcommand{\bOunderbar}{\underline{\bO}}       \newcommand{\bPunderbar}{\underline{\bP}}
\newcommand{\bQunderbar}{\underline{\bQ}}       \newcommand{\bRunderbar}{\underline{\bR}}
\newcommand{\bSunderbar}{\underline{\bS}}       \newcommand{\bTunderbar}{\underline{\bT}}
\newcommand{\bUunderbar}{\underline{\bU}}       \newcommand{\bVunderbar}{\underline{\bV}}
\newcommand{\bWunderbar}{\underline{\bW}}       \newcommand{\bXunderbar}{\underline{\bX}}
\newcommand{\bYunderbar}{\underline{\bY}}       \newcommand{\bZunderbar}{\underline{\bZ}}

\newcommand{\balphaunderbar}{\underline{\balpha}} \newcommand{\bbetaunderbar}{\underline{\bbeta}}
\newcommand{\bgammaunderbar}{\underline{\bgamma}} \newcommand{\bdeltaunderbar}{\underline{\bdelta}}
\newcommand{\bepsilonunderbar}{\underline{\bepsilon}} \newcommand{\bzetaunderbar}{\underline{\bzeta}}
\newcommand{\bfetaunderbar}{\underline{\bfeta}} \newcommand{\bthetaunderbar}{\underline{\btheta}}
\newcommand{\biotaunderbar}{\underline{\biota}} \newcommand{\bkappaunderbar}{\underline{\bkappa}}
\newcommand{\blambdaunderbar}{\underline{\blambda}} \newcommand{\bmuunderbar}{\underline{\bmu}}
\newcommand{\bnuunderbar}{\underline{\bnu}}      \newcommand{\bxiunderbar}{\underline{\bxi}}
\newcommand{\bpiunderbar}{\underline{\bpi}}      \newcommand{\brhounderbar}{\underline{\brho}}
\newcommand{\bsigmaunderbar}{\underline{\bsigma}} \newcommand{\btauunderbar}{\underline{\btau}}
\newcommand{\bupsilonunderbar}{\underline{\bupsilon}} \newcommand{\bphiunderbar}{\underline{\bphi}}
\newcommand{\bchiunderbar}{\underline{\bchi}}    \newcommand{\bpsiunderbar}{\underline{\bpsi}}
\newcommand{\bomegunderbar}{\underline{\bomega}}

\newcommand{\bGammaunderbar}{\underline{\bGamma}} \newcommand{\bDeltaunderbar}{\underline{\bDelta}}
\newcommand{\bThetaunderbar}{\underline{\bTheta}} \newcommand{\bLambdaunderbar}{\underline{\bLambda}}
\newcommand{\bXiunderbar}{\underline{\bXi}}      \newcommand{\bPiunderbar}{\underline{\bPi}}
\newcommand{\bSigmaunderbar}{\underline{\bSigma}} \newcommand{\bUpsilonunderbar}{\underline{\bUpsilon}}
\newcommand{\bPhiunderbar}{\underline{\bPhi}}    \newcommand{\bPsiunderbar}{\underline{\bPsi}}
\newcommand{\bOmegaunderbar}{\underline{\bOmega}}
\endinput
